The Same Only Different: On Information Modality for Configuration Performance Analysis

Configuration in software systems helps to ensure efficient operation and meet diverse user needs. Yet, some, if not all, configuration options have profound implications for the system's performance. Configuration performance analysis, wherein the key is to understand (or infer) the configuration options' relations and their impacts on performance, is crucial. Two major modalities exist that serve as the source information in the analysis: either the manual or source code. However, it remains unclear what roles they play in configuration performance analysis. Much work that relies on manuals claims their benefits of information richness and naturalness; while work that trusts the source code more prefers the structural information provided therein and criticizes the timeliness of manuals. To fill such a gap, in this paper, we conduct an extensive empirical study over 10 systems, covering 1,694 options, 106,798 words in the manual, and 22,859,552 lines-of-code for investigating the usefulness of manual and code in two important tasks of configuration performance analysis, namely performance-sensitive options identification and the associated dependencies extraction. We reveal several new findings and insights, such as it is beneficial to fuse the manual and code modalities for both tasks; the current automated tools that rely on a single modality are far from being practically useful and generally remain incomparable to human analysis. All those pave the way for further advancing configuration performance analysis.

==> Tables/RQ1f1.tex <==
\begin{table}[t!]
\centering

\setlength{\tabcolsep}{0.6mm}
\caption{Identified performance-related options (by manual and code) against the ground truth based on system measurements ($|\mathcal{O}|$ denotes the total number of options; $|\mathcal{O}_m|$ and $|\mathcal{O}_c|$ means the number performance-related options identified from manual and code, respectively. \textbf{Measured} is the number of actual options measured to be indeed performance-related. FP\% and FN\% are the false positive and false negative rates against the ground truth, respectively).}

\label{tb:rq1.1}
\adjustbox{max width=\columnwidth}{
\begin{tabular}{lll|lll|lll}
 \toprule


 \multirow{2}{*}{\textbf{Software}}&\multirow{2}{*}{$|\mathcal{O}|$}&\multirow{2}{*}{\textbf{Measured}}&\multicolumn{3}{c|}{\textbf{Manual}}&\multicolumn{3}{c}{\textbf{Code}}\\

 \cmidrule{4-9}

&&&$|\mathcal{O}_m|$&\textbf{FP\%}&\textbf{FN\%}&$|\mathcal{O}_c|$&\textbf{FP\%}&\textbf{FN\%}\\
 
%\multirow[c]{2}{*}[1pt]{\makecell[c]{Software}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{SUM}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Manual}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Code}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{GT}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{ManualFN}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{CodeFN}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{ManualFP}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{CodeFP}} \\

%  &  &  &  & & & & & \\
 \midrule
\textsc{Httpd} & 77 & 17\% (13/77) & 37 & 38\% (24/64) & 0\% (0/13) & 36 & 41\% (26/64) & 23\% (3/13) \\
\textsc{Lighttpd} & 62 & 27\% (17/62) & 36 & 44\% (20/45) & 6\% (1/17) & 38 & 51\% (23/45) & 12\% (2/17) \\
\textsc{Nginx} & 79 & 6\% (5/79) & 52 & 64\% (47/74) & 0\% (0/5) & 47 & 57\% (42/74) & 0\% (0/5) \\
\textsc{Redis} & 115 & 23\% (26/115) & 81 & 62\% (55/89) & 0\% (0/26) & 75 & 55\% (49/89) & 0\% (0/26) \\
\textsc{MySQL} & 103 & 18\% (19/103) & 72 & 63\% (53/84) & 0\% (0/19) & 68 & 61\% (51/84) & 11\% (2/19) \\
\textsc{HDFS} & 223 & 20\% (45/223) & 112 & 40\% (71/178) & 9\% (4/45) & 84 & 24\% (42/178) & 7\% (3/45) \\
\textsc{MapReduce} & 218 & 18\% (39/218) & 106 & 39\% (70/179) & 8\% (3/39) & 93 & 32\% (58/179) & 10\% (4/39) \\
\textsc{HBase} & 227 & 11\% (25/227) & 74 & 24\% (49/202) & 0\% (0/25) & 64 & 20\% (40/202) & 4\% (1/25) \\
\textsc{Yarn} & 545 & 12\% (66/545) & 176 & 23\% (111/479) & 2\% (1/66) & 141 & 21\% (99/479) & 5\% (3/66) \\
\textsc{Tomcat} & 45 & 20\% (9/45) & 32 & 64\% (23/36) & 0\% (0/9) & 26 & 47\% (17/36) & 0\% (0/9) \\
\midrule
\textbf{Total} & 1694 & 15\% (260/1694) & 778 & 40\% (523/1286) & 3\% (10/338) & 672 & 43\% (422/974) & 5\% (16/338) \\
 \bottomrule
\end{tabular}
}
\end{table}


==> Tables/RQ1f2.tex <==
\begin{table}[t!]
\centering
\caption{Distribution of the causes for false positives/negatives on performance-related options identified by analyzing manual and code.}
\label{tb:rq1.2}
\setlength{\tabcolsep}{0.6mm}
\begin{center}
\adjustbox{max width=\columnwidth}{
\begin{tabular}{llll|ll||lll|ll}
 \toprule
 \multirow[c]{2}{*}[1pt]{\makecell[c]{\textbf{Software}}} & \multicolumn{5}{c||}{\textbf{Manual}} & \multicolumn{5}{c}{\textbf{Code}} \\

\cmidrule{2-11}
 

  &\textbf{FP$_{1}$}&\textbf{FP$_{2}$}&\textbf{FP$_{3}$}&\textbf{FN$_{1}$}&\textbf{FN$_{2}$} &\textbf{FP$_{1}$}&\textbf{FP$_{2}$}&\textbf{FP$_{3}$}&\textbf{FN$_{1}$}&\textbf{FN$_{2}$} \\
 \midrule
\textsc{Httpd}  & 4\% (1/24) & 21\% (5/24) & 75\% (18/24) & 0 & 0 & 4\% (1/26) & 27\% (7/26) & 69\% (18/26) & 0 & 0 \\
\textsc{Lighttpd} & 0\% (0/20) & 5\% (1/20) & 95\% (19/20) & 0 & 0 & 0\% (0/23) & 17\% (4/23) & 83\% (19/23) & 0 & 0 \\
\textsc{Nginx} & 0\% (0/47) & 53\% (25/47) & 47\% (22/47) & 0 & 0 & 0\% (0/42) & 57\% (24/42) & 43\% (18/42) & 0 & 0 \\
\textsc{Redis} & 4\% (2/55) & 35\% (19/55) & 62\% (34/55) & 0 & 0 & 6\% (3/49) & 29\% (14/49) & 65\% (32/49) & 0 & 0 \\
\textsc{MySQL} & 6\% (3/53) & 28\% (15/53) & 66\% (35/53) & 0 & 0 & 4\% (2/51) & 27\% (14/51) & 69\% (35/51) & 0 & 0 \\
\textsc{HDFS} & 3\% (2/71) & 31\% (22/71) & 66\% (47/71) & 0 & 0 & 0\% (0/42) & 36\% (15/42) & 64\% (27/42) & 0 & 0 \\
\textsc{MapReduce} & 3\% (2/70) & 31\% (22/70) & 66\% (46/70) & 0 & 0 & 2\% (1/58) & 36\% (21/58) & 62\% (36/58) & 0 & 0 \\
\textsc{HBase} & 2\% (1/49) & 43\% (21/49) & 55\% (27/49) & 0 & 0 & 0\% (0/40) & 38\% (15/40) & 62\% (25/40) & 0 & 0 \\
\textsc{Yarn} & 0\% (0/111) & 40\% (44/111) & 60\% (67/111) & 0 & 0 & 0\% (0/99) & 39\% (39/99) & 61\% (60/99) & 0 & 0 \\
\textsc{Tomcat} & 0\% (0/23) & 48\% (11/23) & 52\% (12/23) & 0 & 0 & 0\% (0/17) & 47\% (8/17) & 53\% (9/17) & 0 & 0 \\
 \midrule
 
\textbf{Total} & 2\% (11/523) & 35\% (185/523) & 63\% (327/523) & 0\% & 0\%  & 2\% (7/447) & 36\% (161/447) & 62\% (279/447) & 0\%  & 0\%  \\

 \bottomrule
\end{tabular}
}
\end{center}
\end{table}


==> Tables/RQ2f1.tex <==
\begin{table}[ht]
\caption{Discrepancy patterns between performance-related options identified via manual and code.}
\label{tb:rq2}
\centering
\adjustbox{max width=\columnwidth}{

\begin{tabular}{lll|ll}
 \toprule

 \textbf{Software}&\textbf{Manual}&\textbf{Code}&\textbf{Manual Only}&\textbf{Code Only}\\
 

 \midrule
\textsc{Httpd} & 100\% (13/13) & 77\% (10/13) & 23\% (3/13) & 0\% (0/13) \\
\textsc{Lighttpd} & 94\% (16/17) & 88\% (15/17) & 6\% (1/17) & 0\% (0/17) \\
\textsc{Nginx} & 100\% (5/5) & 100\% (5/5) & 0\% (0/5) & 0\% (0/5) \\
\textsc{Redis} & 100\% (26/26) & 100\% (26/26) & 0\% (0/26) & 0\% (0/26) \\
\textsc{MySQL} & 100\% (19/19) & 89\% (17/19) & 16\% (3/19) & 5\% (1/19) \\
\textsc{HDFS} & 91\% (41/45) & 93\% (42/45) & 2\% (1/45) & 4\% (2/45) \\
\textsc{MapReduce} & 92\% (36/39) & 90\% (35/39) & 8\% (3/39) & 5\% (2/39) \\
\textsc{HBase} & 100\% (25/25) & 96\% (24/25) & 4\% (1/25) & 0\% (0/25) \\
\textsc{Yarn} & 98\% (65/66) & 95\% (63/66) & 3\% (2/66) & 0\% (0/66) \\
\textsc{Tomcat} & 100\% (9/9) & 100\% (9/9) & 0\% (0/9) & 0\% (0/9) \\
  \midrule
\textbf{Total} & 96\% (255/264) & 93\% (246/264) & 5\% (14/264) & 2\% (5/264) \\

 \bottomrule
\end{tabular}
}

\end{table}


==> Tables/RQ3f1.tex <==
\begin{table*}[t!]
\centering
%\setlength{\tabcolsep}{0.6mm}
\caption{Distribution of the discrepancy between performance-related dependencies identified via manual and code. $\mathcal{U}$ refers to all unique dependencies; $\Delta${Type} denotes the common dependencies that can be identified from both manual and code but differ according to their types. $|\mathcal{C}|$ denotes the number of options involved in a dependency chain.}
\label{tb:rq3}
\adjustbox{max width=\textwidth}{
\begin{tabular}{llll|lll|ll|ll|ll}
 \toprule


 \multirow{2}{*}{\textbf{Software}}& \multirow{2}{*}{\textbf{Manual}}& \multirow{2}{*}{\textbf{Code}}& \multirow{2}{*}{$\mathcal{U}$}& \multirow{2}{*}{\textbf{Manual Only}}& \multirow{2}{*}{\textbf{Code Only}}& \multirow{2}{*}{$\Delta$\textbf{Type}}&
\multicolumn{2}{c}{\textbf{Mix Option}}&\multicolumn{2}{c|}{\textbf{Perf. Only Option}}&\multicolumn{2}{c}{\textbf{$|\mathcal{C}|\geq3$}}\\

\cmidrule{8-13}

 &&&&&&&\textbf{Manual}&\textbf{Code}&\textbf{Manual}&\textbf{Code}&\textbf{Manual}&\textbf{Code}\\

 \midrule
\textsc{Httpd} & 1 & 4 & 4 & 0\% (0/4) & 75\% (3/4) & 50\% (2/4) & 0\% (0/4) & 75\% (3/4) & 25\% (1/4) & 25\% (1/4) & 25\% (1/4) & 0\% (0/4) \\
\textsc{Lighttpd} & 0 & 2 & 2 & 0\% (0/2) & 100\% (2/2) & 0\% (0/2) & 0\% (0/2) & 100\% (2/2) & 0\% (0/2) & 0\% (0/2) & 0\% (0/2) & 0\% (0/2) \\
\textsc{Nginx} & 4 & 5 & 6 & 17\% (1/6) & 33\% (2/6) & 50\% (3/6) & 33\% (2/6) & 33\% (2/6) & 33\% (2/6) & 50\% (3/6) & 17\% (1/6) & 17\% (1/6) \\
\textsc{Redis} & 9 & 11 & 12 & 8\% (1/12) & 25\% (3/12) & 17\% (2/12) & 25\% (3/12) & 33\% (4/12) & 50\% (6/12) & 58\% (7/12) & 17\% (2/12) & 17\% (2/12) \\
\textsc{MySQL} & 6 & 4 & 6 & 33\% (2/6) & 0\% (0/6) & 0\% (0/6) & 50\% (3/6) & 33\% (2/6) & 50\% (3/6) & 33\% (2/6) & 17\% (1/6) & 0\% (0/6) \\
\textsc{HDFS} & 4 & 7 & 7 & 0\% (0/7) & 43\% (3/7) & 57\% (4/7) & 43\% (3/7) & 57\% (4/7) & 14\% (1/7) & 43\% (3/7) & 29\% (2/7) & 29\% (2/7) \\
\textsc{MapReduce} & 3 & 9 & 9 & 0\% (0/9) & 67\% (6/9) & 33\% (3/9) & 22\% (2/9) & 56\% (5/9) & 11\% (1/9) & 44\% (4/9) & 22\% (2/9) & 33\% (3/9) \\
\textsc{HBase} & 4 & 5 & 6 & 17\% (1/6) & 33\% (2/6) & 67\% (4/6) & 17\% (1/6) & 33\% (2/6) & 50\% (3/6) & 50\% (3/6) & 17\% (1/6) & 17\% (1/6) \\
\textsc{Yarn} & 12 & 11 & 13 & 15\% (2/13) & 8\% (1/13) & 38\% (5/13) & 38\% (5/13) & 38\% (5/13) & 54\% (7/13) & 46\% (6/13) & 31\% (4/13) & 15\% (2/13) \\
\textsc{Tomcat} & 2 & 2 & 2 & 0\% (0/2) & 0\% (0/2) & 0\% (0/2) & 50\% (1/2) & 50\% (1/2) & 50\% (1/2) & 50\% (1/2) & 0\% (0/2) & 0\% (0/2) \\


 \midrule
\textbf{Total} & 45 & 60 & 67 & 10\% (7/67) & 33\% (22/67) & 34\% (23/67) & 30\% (20/67) & 45\% (30/67) & 37\% (25/67) & 45\% (30/67) & 21\% (14/67) & 16\% (11/67) \\
 \bottomrule
\end{tabular}
}
\end{table*}


==> Tables/RQ3f2.tex <==
\begin{table*}[!tp]
\centering
\caption{Dpendency Pattern}

\adjustbox{max width=\textwidth}{
\begin{tabular}{ l l c }
 \toprule
 \multirow[c]{2}{*}[1pt]{\makecell[c]{Pattern}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Descriptions}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Count}} \\
  &  &  \\
 \midrule
 direct-indirect & Manual identifies dependency between two parameters, but not reflected in code & 6 \\
 Yes-No & Whether configuration option is a node in the dependency chain & 14 \\
 Value-Default & Value-Default & 2 \\
 Overwrite-Control & Overwrite-Control & 1 \\
 \bottomrule
\end{tabular}
}


\end{table*}


==> Tables/newRQ2.2-bk.tex <==
\begin{table*}[t!]
\centering
%\setlength{\tabcolsep}{0.6mm}
\caption{Distribution of the discrepancy between performance-related dependencies identified via manual and code. $\Delta${Type} denotes the common dependencies that can be identified from both manual and code but differ according to their types. Other formats are the same as Table [].}
\label{tb:rq2.2}
\adjustbox{max width=\textwidth}{
\begin{tabular}{ll|lllll||lllll}
 \toprule
 \multirow{2}{*}{\textbf{Software}} &  \multirow{2}{*}{\textbf{$\Delta${Type}}}&\multicolumn{5}{c||}{\textbf{Manual}} & \multicolumn{5}{c}{\textbf{Code}} \\

\cmidrule{3-12}

 &&\textbf{$\#$Options}&\textbf{Manual Only}&\textbf{Mixed Options}&\textbf{Perf. Only Options}&$|\mathcal{C}|\geq3$&\textbf{$\#$Options}&\textbf{Code Only}&\textbf{Mixed Options}&\textbf{Perf. Only Options}&$|\mathcal{C}|\geq3$\\

\midrule

\textsc{Httpd} & 2 & 1 & 0\% (0/1) & 0\% (0/3) & 100\% (1/1) & 0\% (0/1) & 3 & 75\% (3/4)) & 100\% (3/3) & 100\% (1/1) & 100\% (1/1) \\
\textsc{Lighttpd} & 0 & 0 & 0\% (0/0) & 0\% (0/2) & 0\% (0/0) & 0\% (0/0) & 2 & 100\% (2/2) & 100\% (2/2) & 0\% (0/0) & 0\% (0/0) \\
\textsc{Nginx} & 3 & 4 & 0\% (1/4) & 100\% (2/2) & 50\% (2/4) & 50\% (1/2) & 2 & 40\% (2/5) & 100\% (2/2) & 75\% (3/4) & 100\% (2/2) \\
\textsc{Redis} & 2 & 9 & 11\% (1/9) & 100\% (3/3) & 67\% (6/9) & 50\% (2/4) & 3 & 27\% (3/11) & 100\% (3/3) & 78\% (7/9) & 100\% (4/4) \\
\textsc{MySQL} & 0 & 6 & 33\% (2/6) & 100\% (3/3) & 100\% (3/3) & 100\% (1/1) & 3 & 0\% (0/4) & 67\% (2/3) & 67\% (2/3) & 100\% (1/1) \\
\textsc{HDFS} & 4 & 4 & 0\% (0/4) & 75\% (3/4) & 33\% (1/3) & 50\% (2/4) & 4 & 43\% (3/7) & 100\% (4/4) & 100\% (3/3) & 100\% (4/4) \\
\textsc{MapReduce} & 3 & 3 & 0\% (0/3) & 40\% (2/5) & 25\% (1/4) & 40\% (2/5) & 5 & 67\% (6/9) & 100\% (5/5) & 100\% (4/4) & 100\% (5/5) \\
\textsc{HBase} & 4 & 4 & 25\% (1/4) & 50\% (1/2) & 75\% (3/4) & 50\% (1/2) & 2 & 40\% (2/5) & 100\% (2/2) & 75\% (3/4) & 100\% (2/2) \\
\textsc{Yarn} & 5 & 12 & 17\% (2/12) & 83\% (5/6) & 100\% (7/7) & 67\% (4/6) & 6 & 9\% (1/11) & 83\% (5/6) & 86\% (6/7) & 100\% (6/6) \\
\textsc{Tomcat} & 0 & 2 & 0\% (0/2) & 100\% (1/1) & 100\% (1/1) & 0\% (0/0) & 1 & 0\% (0/2) & 100\% (1/1) & 100\% (1/1) & 0\% (0/0) \\

\midrule
\textbf{Total} & 23 & 45 & 16\% (7/45) & 64\% (20/31)& 69\% (25/36)& 52\% (13/25)& 15 & 38 & 94\% (29/31)& 83\% (30/36)& 100\% (25/25)\\

 \bottomrule
\end{tabular}
}
\end{table*}


==> Tables/newRQ2.3.tex <==
\begin{table}[t!]
\centering
\caption{Distribution of the causes for false negatives on performance-sensitive dependencies found by analyzing manual and code.}
\label{tb:rq2.3}
%\setlength{\tabcolsep}{0.6mm}
\begin{center}
\adjustbox{max width=\columnwidth}{
\begin{tabular}{lll|ll}
 \toprule
 \multirow[c]{2}{*}[1pt]{\makecell[c]{\textbf{Software}}} & \multicolumn{2}{c||}{\textbf{Manual}} & \multicolumn{2}{c}{\textbf{Code}} \\

\cmidrule{2-5}
 

  &\textbf{FN$_{1}$}&\textbf{FN$_{2}$}&\textbf{FN$_{1}$}&\textbf{FN$_{2}$} \\
 \midrule


  \midrule
\textbf{Total} & 2\% (11/523) & 35\% (185/523) & 63\% (327/523) & 0\%  \\

 \bottomrule
\end{tabular}
}
\end{center}
\end{table}


==> Tables/old/RQ1f1-old.tex <==
\begin{table}[ht!]
\centering
\caption{Perf-sensitive options from code and manual}\label{manualcodegroundtruth}
\adjustbox{max width=\columnwidth}{
\begin{tabular}{ l c c c c c c c c }
 \toprule
\multirow[c]{2}{*}[1pt]{\makecell[c]{Software}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{SUM}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Manual}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Code}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{GT}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{ManualFN}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{CodeFN}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{ManualFP}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{CodeFP}} \\
  &  &  &  & & & & & \\
 \midrule
 httpd & 77 & 37 & 36 & 13 & 0 & 3 & 24 & 26 \\

 lighttpd & 62 & 36 & 38 & 17 & 1 & 2 & 20 & 23 \\

 nginx & 79 & 52 & 47 & 5 & 0 & 0 & 47 & 42 \\

 redis & 115 & 81 & 75 & 26 & 0 & 0 & 55 & 49 \\

 mysql & 103 & 72 & 68 & 19 & 0 & 2 & 53 & 51 \\

 hdfs & 223 & 112 & 84 & 45 & 4 & 3 & 71 & 42 \\

 mapreduce & 218 & 106 & 93 & 39 & 3 & 4 & 70 & 58 \\

 hbase & 227 & 74 & 64 & 25 & 0 & 1 & 49 & 40 \\

 yarn & 545 & 176 & 141 & 66 & 1 & 3 & 111 & 78 \\

 tomcat & 45 & 32 & 26 & 9 & 0 & 0 & 23 & 17 \\
 \bottomrule
\end{tabular}
}
\end{table}


==> Tables/old/RQ2f1-old.tex <==
\begin{table}[ht]
\caption*{Ground truth options discrepancy pattern}
\centering
\adjustbox{max width=\textwidth}{

\begin{tabular}{ l c c c c c c c c c c c c c }
 \toprule
 \multirow[c]{2}{*}[1pt]{\makecell[c]{Software}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Manual}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Code}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Only\\Manual}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Only\\Code}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Both}} \\
  &  &  &  & &  \\
 \midrule
httpd & 13 & 10 & 3 & 0 & 10 \\
 lighttpd & 16 & 15 & 1 & 0 & 15 \\
 nginx & 5 & 5 & 0 & 0 & 5 \\
 redis & 26 & 26 & 0 & 0 & 26 \\
 mysql & 19 & 17 & 3 & 1 & 16 \\
 hdfs & 41 & 42 & 1 & 2 & 40 \\
 mapreduce & 36 & 35 & 3 & 2 & 33 \\
 hbase & 25 & 24 & 1 & 0 & 24 \\
 yarn & 65 & 63 & 2 & 0 & 63 \\
 tomcat & 9 & 9 & 0 & 0 & 9 \\
  \midrule
 SUM & 255 & 246 &14 & 5 & 241 \\
 \bottomrule
\end{tabular}
}

\end{table}


==> Tables/old/RQ3f1-old.tex <==
\begin{table}[t!]
\centering
\caption{Distribution of the discrepancy between performance-related dependencies identified via manual and code.}
\label{tb:rq3}
\adjustbox{max width=\columnwidth}{
\begin{tabular}{ l c c c c c c c }
 \toprule
 \multirow[c]{2}{*}[1pt]{\makecell[c]{Software}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Manual\\Deps}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Code\\Deps}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Unique}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Both in\\Manual Code}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Only in\\Manual}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Only in\\Code}} & \multirow[c]{2}{*}[1pt]{\makecell[c]{Pattern\\Sum}} \\
  &  &  &  & &  &  &  \\
 \midrule
 MySQL & 6 & 4 & 6 & 4 & 2 & 0 & 0 \\
 Lighttpd & 0 & 2 & 2 & 0 & 0 & 2 & 0 \\
 Httpd & 1 & 4 & 4 & 1 & 0 & 3 & 2 \\
 Nginx & 4 & 5 & 6 & 3 & 1 & 2 & 3 \\
 Redis & 9 & 11 & 12 & 8 & 1 & 3 & 2 \\
 Yarn & 12 & 11 & 13 & 10 & 2 & 1 & 5 \\
 HDFS & 4 & 7 & 7 & 4 & 0 & 3 & 4 \\
 Mapreduce & 3 & 9 & 9 & 3 & 0 & 6 & 3 \\
 Hbase & 4 & 5 & 6 & 3 & 1 & 2 & 4 \\
 Tomcat & 2 & 2 & 2 & 2 & 0 & 0 & 0 \\
 \bottomrule
\end{tabular}
}
\end{table}


==> sections/old/method.tex <==
\section{Methodology}
\label{methodology}




\subsection{Overview of the Study Protocol}

\input{Tables/software}


\subsection{Software Systems}

%latest stable version

To collect data from widely-used configurable systems, we study those open-sourced ones that also come with well-documented manuals. The list has been illustrated in Table []. We can clearly see that the systems studied come from diverse domains, with different languages and complexity, while being widely used by the community. To ensure the validity of the system, we take the latest stable version of each system and analyze its code and the corresponding manual by the date of analysis, i.e., Sep 2023. This is reasonable as it represents the most stable state of a system without being affected by the new releases that are known to be issue-prone.


\subsection{Identifying Performance-related Options}




\subsubsection{Manual Analysis}


Two authors who are experienced software engineers independently analyzed the manual to identify performance-related options. This follows a mix of blacklist and whitelist approaches []. The blacklist contains several keywords that, if detected in the manual's description, would cause the corresponding option to be eliminated immediately. In contrast, if a description contains any of the terms in the whitelist, then the corresponding option is considered performance-related. The procedure is as follows:


\begin{enumerate}
    \item \textbf{Screening:} As shown in Table, we conduct an initial screening by identifying the keywords for blacklist and whitelist. The former involves terms about resource names, path information, and functional needs, which are clearly non-performance-related. The latter, in contrast, contains those that describe system memory, operating modes, thread control, etc.
    \item \textbf{Blacklist Exclusion:} We eliminate any options which have descriptions that contain the keywords in the blacklist. By the end of this phase, the two authors exchange their filtered list and any disagreement would be discussed or consulting the other author or external expert until a consensus can be made.
    \item \textbf{Whitelist Inclusion:} In the remaining options, the description of which contains any of the terms in the whitelist is said as performance-related. Again, extensive discussions were taken place to resolve any disagreement in the end. 
    \item The two authors that independently and manually read and understand the renaming options and pick the performance-related ones as understood from the description. A final list is shared and discussed until agreements are reached. The same process is repeated for the manual of every system studied.
\end{enumerate}

For example, on the system ?, is an option that was filtered out during the stage of using the blacklist, because ???; similarly, is an option that is included when analyzing the manual via whitelist since ??. \textcolor{red}{Hongyuan, please complete the above example}



\subsubsection{Code Analysis}

To understand the performance-related options from code, we leverage a semi-automated approach that relies on modern taint analysis tools. Again, the two authors who are experienced software engineers took the lead, and all authors were involved in the following procedure:

\begin{enumerate}
    \item \textbf{Operation Categorization:} We at first define any operation and function that belong to the following categories are performance sensitive, \textcolor{red}{Hongyuan, add concrete example for each}:
    \begin{itemize}
         \item Memory operations, including array or stack allocations.
        \item Cache operations, including high-frequency cache updates or cache synchronization.
        \item I/O operations, e.g., those accessing the persistent storage.
        \item Threading process, such as thread start/stop operations and the creation of threads or thread pools.
        \item Loop operations, including for, while, and do-while loops.
        \item Network communication, \textcolor{red}{Hongyuan, add example}.
        \item Error control process, \textcolor{red}{Hongyuan, add example}..
    \end{itemize}
    Those categories are discussed among all authors until an agreement has been reached.


   \item \textbf{Variable Identification:} It is easy to understand what the configuration options are by reading the configuration file, e.g., \texttt{yaml} files. Yet, since the configuration options in the code are codified in different ways depending on the systems, we use the different approaches below to establish the mappings between configuration options and the corresponding variables in the code:
    \begin{itemize}
        \item \textbf{Unified Analysis}: For systems like \textsc{MySQL}, \textsc{Lighttpd}, \textsc{Nginx}, and \textsc{Redis}, the variables for configuration options are centrally organized in a single file with identical names, and hence the mappings can be found directly.
        \item \textbf{Segmented Analysis}: For \textsc{Httpd} and \textsc{Tomcat}, the variables are written in separate source code files but they are still centrally involved in a \textsc{main} thread. For those, we analyze the control flow to find the relevant code files and the corresponding variables. 
        \item \textbf{Scattered Analysis}: For \textsc{HDFS}, \textsc{MapReduce}, \textsc{HBase}, and \textsc{YARN}, the variables are also distributed across the codebase and they are only called on-demand. Yet, those variables are all accessible via the \texttt{setter()} and \texttt{getter()} function. Therefore, we analyze each of the \texttt{setter()} and \texttt{getter()} in the source code to identify the corresponding variables.
    \end{itemize}
   Again, the two lead authors conduct the analysis independently and exchange the results in the end to reach a consensus. 
   
  
    \item \textbf{Taint Analysis:} To extract those performance-related options by analyzing the code, we leverage taint analysis, where we use variables identified serve as the sources and the performance-sensitive operations are the sink. For C/C++ systems, we use \textsc{Llmast}, and for Java systems, we use \texttt{JavaParser} []. We say an option is performance-related if it fits with either case below:

    \begin{itemize}
        \item In the \textbf{top-down manner}, the taint analysis would procedure some taint flows that indicate which performance-sensitive operations would interact with the variables identified. However, it is unclear whether those variables can impact the behavior of the operation. To confirm that point, we further extract the corresponding code fragments from the Abstract Syntax Tree to investigate whether the execution path between the variables identified and performance-related operations involve logical operators, e.g., \texttt{If/Else} or \texttt{While}. If that is the case, we find a performance-related option/variable.

        \item We also follow a \textbf{bottom-up} approach starting from each of the performance-sensitive operations, based on which we identify the parameters that are part of the variables found. We then use taint analysis to trace back to the origin of those parameters to confirm their interaction. If an interaction exists, the corresponding variable is performance-related.
    \end{itemize}
\end{enumerate}



\subsubsection{System Measurement (Ground Truth)}

To identify the ground truth, we manually change each configuration option and examine whether such a change leads to significant performance deviation. This is achieved by running and profiling each system under its standard benchmark, which is a common procedure that is widely used in the community []. 

For each option, we sample two possible values as the representatives (excluding the default): for the numeric options, we use the maximum and minimum within the range documented. If no range is provided, we use the positive upper limit as the maximum value and 0 as the minimum value. For boolean options, we simply flip their \texttt{true} and \texttt{false}. For other enumerate options, we compare all pairs of the possible values in the eligible range. For all cases, we compare the performance achieved by setting the two values of an option, while keeping the other options with their default values.

We repeat the process five times to ensure the stability and reliability. A numeric or boolean option is said to be indeed performance-related if the average performance of setting one value can have more than $5\%$ deviation compared with that of the setting the said option with the other value; an enumerate option is performance-related if the average performance of any pair of its value has deviation greater than $5\%$. It is worth noting that the above is a typical setting being acknowledged as a de facto standard in the field []. 



\subsection{Extracting Dependencies}


Once the performance-related options have been identified, we then seek to extract performance-related dependencies using manual or code individually. We say a dependency is performance-related if at least one of its options involved is a performance-related option.

\subsubsection{Dependencies by Manual}


To extract performance-related dependencies from the manual, two authors independently perform the following:

\begin{enumerate}
    \item The non-performance-related options and their descriptions are filtered out.
    \item Each author read and analyzed the description of each option remaining. An option is said to have a dependency on the other if its description has clearly mentioned the other option.
    \item In the end, both lead authors combined the list of dependencies identified, and they were discussed among all authors for cross-checking and verification. This includes, but is not limited to, checking the accuracy, completeness, and logical relationships between the descriptions and the related configuration options.
    \item The above process was repeated by two rounds of rigorous review to mitigate bias.
\end{enumerate}

The extracted dependencies represent the information that can be obtained by analyzing the manual.




\subsubsection{Dependencies by Code}


To extract dependency information from the code, we again focus on the performance-related options only. We then apply taint analysis using the same aforementioned tools, such that the variable of a performance-related option serves as the source while that of the other performance-related option is the sink. Within the results, we check whether there is a call path that involves both variables. If that is the case, we investigate the code segment and examine if both variables are involved in some form of logical operation, such as \texttt{If/Else}, \texttt{Switch}, or \texttt{While} loop.

Two authors independently execute the above process, and the final results are discussed and agreed on amongst all authors.





\subsection{Software Systems}
We examined 10 widely-used open-source software systems, five written in CPP and five in JAVA.

The five widely-used CPP-based software systems are MySQL, Nginx, Redis, Lighttpd, and Httpd. These software systems are extensively applied jiuin database management, web servers, and data storage. MySQL is a popular relational database management system. Nginx is a high-performance web server and reverse proxy server. Redis is an in-memory data structure store that supports various data structures. Lighttpd is a lightweight web server. Httpd (Apache HTTP Server) is a widely-used web server.

The five JAVA-based open-source software systems are HDFS, MapReduce, HBase, YARN, and Tomcat. These systems play significant roles in big data processing and web application deployment, widely applied in distributed computing, data storage, and application servers. Specifically, HDFS is a scalable distributed file system. MapReduce is a distributed, parallel processing framework. HBase is a distributed database running on HDFS. YARN is a resource management and job scheduling framework within the Hadoop ecosystem. Tomcat is a popular Java Servlet and JavaServer Pages container.

\subsection{Data Collection}
In this section, we first briefly introduce how we collected performance-related configuration information and dependency information from source code and software manuals, and then describe the workflow steps in each subsection.

Our workflow is sufficiently general to adapt to software systems of different languages and environments. Figure workflow illustrates an overview of our workflow, which is mainly composed of two parts: 1) manual analysis and 2) code analysis. Manual analysis involves examining configuration option names and descriptions to determine if they are related to performance. Code analysis identifies performance-sensitive operations and the locations of configuration variables in the code to determine if configuration options might be performance-related.

\begin{figure*}[htb] 
    \centering 
    \includegraphics[width=\textwidth]{Figures/PerfCodeSearch.png}
    \caption{Perfsearch} 
    \label{fig:example} 
\end{figure*}

\subsubsection{Perf Knobs Selection}

\paragraph{Code}

\begin{enumerate}
    \item Identify performance-related operations. We identified five types of performance-related operations:
    \begin{enumerate}
        \item Memory operations, including array or stack allocations.
        \item Cache operations, including high-frequency cache updates or cache synchronization.
        \item I/O operations.
        \item Thread operations, such as thread start/stop operations and the creation of threads or thread pools.
        \item Loop operations, including for, while, and do-while loops.
    \end{enumerate}
    For each software, we found the classes or functions that actually perform these operations. For instance, in MySQL, the \texttt{setup\_io\_cache} function is used to set pointers for I/O cache, which we classify as I/O-related and cache-related operations.
    
    \item Locate the positions of configuration variables in the software code. First, we determined the configuration reading and storage methods for each software to establish a mapping relationship between configuration options and variables. We categorized the 10 software systems based on their configuration reading methods:
    \begin{enumerate}
        \item Unified reading: MySQL, Lighttpd, Nginx, and Redis fall into this category, where the software reads all configuration information at startup and stores it in the corresponding memory space for subsequent system calls.
        \item Segmented reading: Includes Httpd and Tomcat, where the software reads configuration information in modules when the respective module is invoked.
        \item Scattered reading: Includes HDFS, MapReduce, HBase, and YARN, where these software systems use the \texttt{get()} function to read configuration values when calling the respective configuration variables.
    \end{enumerate}
    We organized the configuration reading and storage methods for all 10 software systems and established a mapping relationship from configuration files to configuration variables.
    
    \item Check if configuration variables in the code have control dependencies with performance-related operations. First, we consider configuration variables as sources and performance-related operations as sinks, using taint analysis to trace the taint flow of each configuration variable. We analyze whether there is an execution path dependency between the configuration variables and performance-related operations. If such a dependency exists, the corresponding configuration may impact software performance.
\end{enumerate}





\paragraph{Manual}

\begin{enumerate}
    \item We perform initial screening of performance configurations using blacklists and whitelists of keywords. First, we define a set of keywords that might indicate performance issues, forming a blacklist. These keywords may include ``proxy,'' ``path,'' ``port,'' etc. Through blacklist screening, we can exclude configuration items unrelated to performance. Next, we define a set of keywords related to performance, forming a whitelist. These keywords may include ``cache,'' ``size,'' ``block,'' etc. In the configuration items remaining after blacklist screening, we use the whitelist keywords for further screening to identify the configuration items most likely related to performance. Subsequently, the screened configuration items are reviewed manually by an expert team to further confirm whether these configurations are indeed performance-related, ensuring the accuracy and validity of the screening results. Through this method, we can efficiently identify key configuration items that impact system performance.
\end{enumerate}

\paragraph{Ground Truth}

First, we set the system configurations to their default values and run the system for baseline performance testing, recording various performance metrics such as response time, throughput, CPU usage, memory usage, I/O operation time, etc. Next, we adjust each configuration item to its minimum value, run the system again, and record the performance metrics under these configurations. Finally, we set the configuration items to their maximum values and conduct the same performance tests and data recordings to observe the system's performance under maximum configuration conditions.

For each configuration value, we run the system five times to ensure the stability and reliability of the test results. All performance data will be recorded and analyzed in detail to compare the impact of default, minimum, and maximum configurations on system performance. Through these tests, we can determine which configuration items significantly affect system performance under different settings.




\subsubsection{Configuration Dependency}

\paragraph{Code}

\begin{enumerate}
    \item First, we utilize taint analysis where the source is the declaration of configuration variables, and the sink is the invocation or declaration of other configuration variables. This allows us to trace the taint flow of configuration variables and identify code segments where there is an execution path dependency with other configuration variables. After extracting the relevant code segments, two expert teams will conduct a manual review to determine whether there is an execution path dependency between the configuration items and document the specific dependencies. Finally, the results from both teams will be cross-verified.
\end{enumerate}

\paragraph{Manual}

\begin{enumerate}
    \item We search the manual documents for descriptions of each configuration item to identify any mentions of other configuration items. All descriptions that include the names of other configuration items will be filtered out. These descriptions will then be manually reviewed by two expert teams, who will cross-verify their findings.
\end{enumerate}



==> sections/old/rq1.tex <==
\section{Empirical Study Results}


%\subsection{RQ1: Mismatching against Ground Truth}
\subsection{RQ1: Performance-related Options}

\input{Tables/newRQ1.1}
\input{Tables/newRQ1.2}
\input{Tables/newRQ1.3}

\subsubsection{Operationalization}

%Given the options measured to be indeed performance-related serving as the ground truth, 

Since there is no guarantee that the options identified via either manual or code analysis are indeed performance-related, we use the measured results as the ground truth, i.e., we say an option is performance-related only if adjusting it can change the performance by more than $5\%$. In this way, we report on the true positive rate, false positive rate, and false negative rates of the results obtained by analyzing the manual and code.


To study the discrepancy of correctly identifying performance-related options by using manual and code individually, we use the following patterns observed:

\begin{itemize}
    \item \textbf{Manual Only:} This refers to the true performance-related options (against ground truth) that are found by studying the manual only rather than code.
    \item \textbf{Code Only:} In contrast, this refers to the true performance-related options (against ground truth) that are identified via analyzing the code but are not noticeable from the manual.
\end{itemize}



To further understand why analyzing manual or code alone might lead to some false results, we analyze the in-depth reasons that result in the errors; for false positive cases, we summarize the  causes below:

\begin{itemize}
    \item \textbf{FP}$_1$: The configuration option is completely discarded. However, this might not be noticeable in the manual (since it might not have been mentioned) or code (since the call graph can be complicated).
    
    \item \textbf{FP}$_2$: The option has no implication on the performance at all, i.e., the performance stays the same before and after the change.
    
    \item \textbf{FP}$_3$: The impact of the configuration option on performance is minimal. That is to say, there is indeed a performance drop/improvement after the change, but the magnitude is less than $5\%$.
\end{itemize}

Similarly, for false negative cases, we draw on the categories below:

\begin{itemize}
    \item \textbf{FN}$_1$: There is indeed a significant performance implication but the option is rather complicated and can be hardly identified via manual or code analysis. For example, its description is highly ambiguous in the manual and the code involves many invocations to external APIs.
    \item \textbf{FN}$_2$: The performance implication of the options only marginally beyond $5\%$, e.g., by less than $1\%$, and it is possibly due to randomness in the execution. Yet, for the sake of completeness, we classify these as performance-related options too.
\end{itemize}

\subsubsection{Findings}

In this section, we will describe in detail how to determine if configurations are related to performance based on information from manuals and code.

\subsection{Select Knobs from Manual}
The manuals provided by the software's official personnel contain numerous explanations on how configuration options affect the software's operation. By reading these explanations, we can determine how configuration options impact software performance. Manually studying all configurations is very time-consuming, so we adopt a keyword-based blacklist and whitelist approach to quickly filter out configuration knobs that may affect software performance.

Our blacklist keywords include information about resource names, path information, etc. (e.g., examples). We perform an initial screening of software configuration names and descriptions using the blacklist keywords. For configurations containing blacklist keywords, two experienced software engineers independently judge whether they are performance-related. If they are performance-related, the configuration is added back to the configuration set for the next whitelist screening step. After the blacklist screening, we obtained the data.

Our whitelist keywords include keyword groups related to system memory, operating modes, thread control, etc. (e.g., examples). We search the configuration options filtered out by the blacklist in the previous step using the whitelist keyword groups. If a configuration contains whitelist phrases, we consider it potentially performance-related. Similarly, after the initial whitelist screening, two experienced software engineers independently judge the configurations that do not contain whitelist keywords. Based on their judgments, we decide whether to add them to the performance-related configuration set. After this step, we obtained the data.

\subsection{Select Knobs from Code}
First, we need to identify performance-related operations in each software. As shown in the figure, we define seven types of performance-expensive operations: (1) memory-related operations, (2) cache-related operations, (3) I/O-related operations, (4) thread operations, (5) loop operations, (6) network communication operations, and (7) error control operations. In each software, we locate the classes or functions that actually execute these operations, including basic language operations like java.io and unique performance-expensive operations specific to each software. The results of the five types of performance-expensive operations in each software are summarized in the table.

We established a mapping relationship from configuration files to configuration variables. For software with unified and segmented reading types, we established a correspondence between configuration variable names and configuration option names. For software with scattered reading types, we established a correspondence between configuration option names and configuration abbreviations (e.g., examples).

Next, we use taint analysis to check whether configuration variables in the code have control relationships with performance-related operations. For C++ software, we use [specific tool], and for Java software, we use JAVAPARSER. We consider two types of control relationships: 1. There is an execution path dependency between the configuration and performance-related operations. To search for this relationship, we use the invocation of configuration variables as the source (if it is a get function call, the received variable is the source), and the software's performance-related operations as the sink. We determine whether each software's taint flow contains performance-related operations. If the taint flow contains performance-related operations, we extract the corresponding code fragments and AST syntax trees for further analysis to determine whether there is an execution path dependency between the configuration variables and performance-related operations. If there is an execution path dependency, as in the example, we consider the corresponding configuration may affect software performance. We obtained a certain number of parameters belonging to the first category for further research. 2. The invocation statement of the configuration variable is part of the performance-related operation's code. We use taint analysis to locate the variables of performance-related operations in the code and check whether they are within the code range of the performance-related operations, further determining whether the configuration and performance operations satisfy the second type of control relationship.

\subsection{Select Knobs from Ground Truth}
For each software system, we use standard benchmark programs for performance testing, running our tests on a configured computer. Table 2 shows the benchmark programs for each software.

For numeric values, we use the maximum, minimum, and default values within the range if provided in the manual. If no range is provided, we use the positive upper limit of the data type as the maximum value and 0 as the minimum value. For boolean data, we use true and false. For set types, we select three different values. For other special types, we select values that are as different as possible. The table shows our selected values for each data type.

We run the system five times under each configuration value to ensure the stability and reliability of the test results. All performance data will be recorded and analyzed in detail to compare the specific impact on system performance. If the performance change between any two values of the same configuration is greater than 5\%, it is considered to have a significant impact on performance. If the impact on performance is between 1-5\%, it is considered to potentially affect performance under certain workloads. Through these tests, we can determine the extent to which configuration items affect system performance.

\subsection{Discrepancy Pattern}
We observed detailed phenomena regarding the inconsistencies in the performance impact of software configurations from manuals, code, and actual runtime. Firstly, the accuracy of determining performance-related configuration options through code is higher than through manuals. Secondly, the performance-related operations that cause the most false positives in code are exception controls. Based on the ground truth results, we categorized the false positives into three patterns: 1. The configuration option is no longer effective. 2. During actual execution, the configuration option did not impact performance. 3. The configuration option's impact on performance is minimal and may only be significant under specific workloads. The most frequent pattern is the third one, with 294 instances from manual judgments and 279 from code judgments.
%\input{Tables/old/RQ1f1-old}
\input{Tables/RQ1f1}

%\input{Tables/RQ1f2}

==> sections/old/rq2.tex <==
\subsection{RQ2: Performance-related Dependencies}


\input{Tables/newRQ2.1}

\input{Tables/newRQ2.2}

\subsubsection{Operationalization}


We collect all the performance-related dependencies identified via manual/code and further confirm they are valid via manual code analysis. We hence found that all the dependencies identified are indeed present and performance-related, from which the unique dependencies for each system are reported. Yet, we observe the following patterns between those obtained via manual and code:

\begin{itemize}
    \item \textbf{Manual Only:} There exist performance-related dependencies that are only clearly observable in the manual but deeply hidden in the code.
    \item \textbf{Code Only:} Similarly, certain performance-related dependencies have not been mentioned in the manual at all but clearly noticeable in the code.
\end{itemize}


For a given dependency, we found two possible styles:

\begin{itemize}
    \item \textbf{Mixed Options:} This means one of the options involved is not relevant to performance.
    \item \textbf{Performance Only Options:} This refers to both options in the dependencies that are performance-related.
\end{itemize}
We report on the styles as identified by manual and code, respectively.


In addition, we also analyze the number of options involved in a dependency chain, which is a direct reflection of the dependency of complexity for a system. Again, we showcase how those complex dependency chains, i.e., the number of options greater than 3, can be detected via manual and code analysis individually.

Since some performance-related dependencies can only be identified in manual not code (and vice versa), we also study why certain dependencies have been missed according to the following reasons:

\begin{itemize}
    \item \textbf{Missing}$_1$:
    \item \textbf{Missing}$_2$:
\end{itemize}


\subsubsection{Findings}


\subsection{RQ2}



This is an overview of the situation. Among all the results where ground truth indicates a positive impact on performance, there are 19 configurations predicted as negative by the manual. In other words, when using the manual to judge performance relevance, these configurations were incorrectly determined to be performance-irrelevant. Correspondingly, we also compared the code prediction results with ground truth and found that there are 9 configurations where the code prediction resulted in false negatives (FN).

For the above results, we categorized them based on the data types of the configurations in the manual and the performance-sensitive operations in the code, as shown in Table 5.1. We found that although the number of false negatives when using code to determine if a configuration is performance-relevant is lower than when using the manual, in the CodeFN cases, the most frequent performance operation is error handling. Combining with the results of RQ1, we found that error handling operations often provide more warning information and are less likely to be triggered under regular benchmark tests.
\input{Tables/RQ2f1}

==> sections/old/rq3.tex <==
\subsection{RQ3: Challenges for Current Tools}


\subsubsection{Operationalization}

From those performance-related options and dependencies identified using manual or code, we then seek to investigate the effectiveness of existing tools that are designed to automatically predict them. In particular, we choose state-of-the-art tools for performance-related options inference and dependencies identification, each of which relies on the information extracted from manual or code individually. The former involves:

\begin{itemize}
    \item \textbf{\texttt{SafeTune}:} As a representative that relies on information from the \textbf{manual}, \texttt{SafeTune} identifies performance-related options by modeling and analyzing configuration documentation.
    \item \textbf{\texttt{DiagConfig}:} In contrast, \texttt{DiagConfig} trains a Random Forest to predict whether the given configuration option and its associate code snippet are performance-related. As such, it uses \textbf{code} as the main source of information.
\end{itemize}


The latter also includes two representatives:

\begin{itemize}
    \item \textbf{\texttt{GPTuner}:} \texttt{GPTuner} leverages the understanding capabilities of large
language models to infer dependencies by reading the texts from the \textbf{manual}. It is designed for inferring any dependencies.
    \item \textbf{\texttt{CDep}:} In \texttt{CDep}, the dependencies are predicted by analyzing the \textbf{code} using rule mining. Again, it can be used for any dependencies beyond the performance-related ones.
\end{itemize}
Since those tools are cross-project in nature, e.g., the code/manual learned from one project is directly exploited for predicting in the target project, we use all the manual/code that exists in a target project as the testing data. We choose the common metrics, i.e., recall, precision, and F1 score in the evaluation as they are robust to data imbalance [].

Note that, all tools are stochastic in nature except \texttt{CDep}, therefore for those, we repeat ? runs and reports on the deviation as necessary.

\subsubsection{Findings}



\begin{figure}[t!]
\centering
\subfloat[\texttt{SafeTune} (manual)]{\includestandalone[width=0.49\columnwidth]{Figures/rq4-3}}
~\hfill
\subfloat[\texttt{DiagConfig} (code)]{\includestandalone[width=0.49\columnwidth]{Figures/rq4-4}}

\caption{Effectiveness of tools that predict performance-related options over ? runs.}
\label{fig:rq4-1}
\end{figure}


\begin{figure}[t!]
\centering
\subfloat[\texttt{GPTuner} (manual)]{\includestandalone[width=0.49\columnwidth]{Figures/rq4-1}}
~\hfill
\subfloat[\texttt{CDep} (code)]{\includestandalone[width=0.49\columnwidth]{Figures/rq4-2}}

\caption{Effectiveness of tools that predict configuration dependencies over ? runs.}
\label{fig:rq4-2}
\end{figure}


\subsection{RQ3}


\subsection{Knobs Dependency Search in Code}
The code search process utilizes taint analysis methods. For Java programs, we use the javaparser library, and for C++ programs, we use the llmast tool. Our search strategy is to find the taint flow of configuration variables in the code and look for calls to other configuration variables within the taint flow. Here, the source of the taint analysis is the declaration of the configuration variable, and the sink is the calls or declarations of other configuration variables. If the taint flow includes calls to other variables, we check whether there is a control-flow dependency between the two configuration variables (here, we define control-flow statements as those affecting the data flow in the code, such as loop, switch, while, if, etc.). If such a dependency exists, we mark this segment of the code. Next, two groups of expert teams manually review these marked code locations to capture the control-flow dependency between configuration items and record the specific relationship between the two configuration variables. (Example)

\subsection{Knobs Dependency Search in Manual}
During the detailed document review process, the manual needs to be carefully read, analyzing the detailed descriptions of each configuration item word by word. Particular attention should be paid to descriptions that mention the names of other configuration items, as they may reveal interdependencies or associations between configuration items. Once such descriptions are found, they should be recorded and categorized.

Next, these filtered descriptions are submitted to two groups of expert teams. Each team consists of senior experts in the field who will conduct in-depth manual reviews of these descriptions. This includes, but is not limited to, checking the accuracy, completeness, and logical relationships between the descriptions and the related configuration items. Additionally, the expert teams need to assess whether these descriptions help users better understand and use the configuration items.

After each team completes their review, their results need to be compared and cross-checked. Ultimately, through two rounds of rigorous review and cross-checking, we will obtain a detailed and accurate list of configuration item descriptions.

\subsection{Dependency Discrepency Pattern}
We compared the collected dependencies and found some notable phenomena. Finding:
1. Some configuration dependencies can form a chain of configuration dependencies. We consider a chain to be a dependency relationship involving more than three configuration options. Across all 10 software systems, we found a total of XXX chains, of which XXX include performance-related configuration options. The longest chain contains XXX configuration options.
2. There are many inconsistencies in the types of configuration dependencies collected from manuals and code. We will elaborate on the classification of these inconsistencies in the following content.

\input{Tables/RQ3f2}
\input{Tables/RQ3f1}

Dependency Classification:
We first classified the configuration relationships. Based on previous work, we classified the configuration dependencies according to three criteria:
1. Functional configuration dependency [Cdep]
2. Whether the relationship between two configurations is direct or indirect
3. Whether it is a node in a chain

We categorized the inconsistencies exhibited in the classification of configuration dependencies from manuals and code into mismatch categories. We identified six Discrepancy Patterns of dependencies as shown in the figure below:
1. Direct-indirect inconsistency: One source of information shows a direct relationship, while the other shows an indirect relationship.
2. In-chain vs. not-in-chain: Whether the dependency belongs to a chain in the dependencies extracted from the manual and code respectively.
3. Numerical relationship vs. default relationship: The configuration dependencies extracted from the manual and code belong to numerical relationships and default relationships respectively.
4. Coverage relationship vs. control relationship: The configuration dependencies extracted from the manual and code belong to coverage relationships and control relationships respectively.



==> sections/old/rq4.tex <==
\subsection{RQ4: Challenges for Current Tools}


\subsubsection{Operationalization}


\subsubsection{Findings}



\subsection{RQ4}
In this section, we compare our collected experimental results with four state-of-the-art approaches. These four approaches use either code information or manual information to determine whether configuration options are performance-related and the dependencies between configuration options. Their details are listed in Table 7.1.

\subsection{Performance Knobs Selection}
SafeTune identifies performance-sensitive options by modeling and analyzing system configuration-related documents. DiagConfig determines this by tracking perf-sensitive operations in Java code and establishing a random forest model. We applied these two tools to our software system for sensitive configuration options identification.

\textbf{Results Analysis:} \texttt{SafeTune} identified 641 performance-sensitive options out of a total of 778 configuration options. Among them, 248 options significantly impacted system performance (greater than 5:\%) in the ground truth test, with an accuracy of 38.7:\%. \texttt{DiagConfig} selected 161 performance-sensitive options out of 500 configuration options, with an accuracy of 15.0:\%. \texttt{DiagConfig} did not exhibit the expected accuracy advantage of using code information. The detailed results for each software are presented in Table 7.2.

\subsection{Configuration Dependency}
Gptuner leverages the understanding capabilities of large language models and its knowledge to infer dependencies between configurations. \texttt{Cdep} identifies dependencies by recognizing specific patterns in the code and categorizes these relationships. We compared the results of these two tools with our results.

\textbf{Results Analysis:} \texttt{Gptuner} identified 160 configuration dependencies out of a total of 235 options that significantly impacted system performance (greater than 5:\%) in the ground truth test, with an accuracy of 31.9:\%. \texttt{Cdep} selected 70 configuration dependencies out of 151 configuration options, with an accuracy of 32.9:\%. The detailed results for each software are presented in Table 7.3.

% \input{Tables/RQ4f2}
% \input{Tables/RQ4f4}
% \input{Tables/Gptuner}

% \input{Tables/Safetune}


